Role of Non-Ideal Dissipation with Heating-Cooling Misbalance on the Phase Shifts of Standing Slow Magnetohydrodynamic Waves

We analyse the phase shifts of standing, slow magnetohydrodynamic (MHD) waves in solar coronal loops using a linear MHD model taking into account the role of thermal conductivity, compressive viscosity, radiative losses, and heating-cooling misbalance. We estimate the phase shifts in time and space of density and temperature perturbations with respect to velocity perturbations and also calculate the phase difference between density and temperature perturbations. The overall significance of compressive viscosity is found to be negligible for most of the loops considered in the study. For loops with high background density and/or low background temperature, the role of radiative losses (with heating-cooling misbalance) is found to be more significant. Also the effect of heating-cooling misbalance with a temperature- and density-dependent heating function is found to be more significant in the case of longer loop lengths ($L=500$\, Mm). We derived a general expression for the polytropic index [$\gamma_{\rm eff}$] and found that under linear MHD the effect of compressive viscosity on polytropic index is negligible. The radiative losses with constant heating lead to a monotonic increase of $\gamma_{\rm eff}$ with increasing density whereas the consideration of an assumed heating function [$H(\rho,T) \propto \rho^{a}T^{b}$, where $a=-0.5$ and $b=-3$] makes the $\gamma_{\rm eff}$ peak at a certain loop density. We also explored the role of different heating functions by varying the free parameters $a$ and $b$ for a fixed loop of $\rho_0 = 10^{-11}$\, kg $\text{m}^{-3}$, $T_0 = 6.3$\, MK and loop length $L= 180$\, Mm. We find that the consideration of different heating functions [$H(\rho,T)$] leads to a significant variation in the phase difference between density and temperature perturbations; however, the polytropic index remains close to a value of 1.66.

==> sola_example_labels.tex <==
This file contains the command names and the labels used in
the associated .tex file.    It is useful to have present file open
as the same time of the .tex file to copy/paste definitions.
When a new definition is added, it is important to keep this file
updated. 

   % Copy/paste of the definitions used in the .tex
\newcommand{\BibTeX}{\textsc{Bib}\TeX}
\newcommand{\etal}{et al.}

% Definitions for equations
\newcommand{\deriv}[2]{\frac{{\mathrm d} #1}{{\mathrm d} #2}}
\newcommand{\rmd}{ {\ \mathrm d} }
\renewcommand{\vec}[1]{ {\mathbf #1} }
\newcommand{\uvec}[1]{ \hat{\mathbf #1} }
\newcommand{\pder}[2]{ \f{\partial #1}{\partial #2} }
\newcommand{\grad}{ {\bf \nabla } }
\newcommand{\curl}{ {\bf \nabla} \times}
\newcommand{\vol}{ {\mathcal V} }
\newcommand{\bndry}{ {\mathcal S} }
\newcommand{\dv}{~{\mathrm d}^3 x}
\newcommand{\da}{~{\mathrm d}^2 x}
\newcommand{\dl}{~{\mathrm d} l}
\newcommand{\dt}{~{\mathrm d}t}
\newcommand{\intv}{\int_{\vol}^{}}
\newcommand{\inta}{\int_{\bndry}^{}}
\newcommand{\avec}{ \vec A}
\newcommand{\ap}{ \vec A_p}
\newcommand{\bb}{ \vec B}
\newcommand{\jj}{ \vec j}
\newcommand{\rr}{ \vec r}
\newcommand{\xx}{ \vec x}

% Definitions for the journal names
\newcommand{\adv}{    {\it Adv. Space Res.}} 
\newcommand{\annG}{   {\it Ann. Geophys.}} 
\newcommand{\aap}{    {\it Astron. Astrophys.}}
\newcommand{\aaps}{   {\it Astron. Astrophys. Suppl.}}
\newcommand{\aapr}{   {\it Astron. Astrophys. Rev.}}
\newcommand{\ag}{     {\it Ann. Geophys.}}
\newcommand{\aj}{     {\it Astron. J.}} 
\newcommand{\apj}{    {\it Astrophys. J.}}
\newcommand{\apjl}{   {\it Astrophys. J. Lett.}}
\newcommand{\apss}{   {\it Astrophys. Space Sci.}} 
\newcommand{\cjaa}{   {\it Chin. J. Astron. Astrophys.}} 
\newcommand{\gafd}{   {\it Geophys. Astrophys. Fluid Dyn.}}
\newcommand{\grl}{    {\it Geophys. Res. Lett.}}
\newcommand{\ijga}{   {\it Int. J. Geomagn. Aeron.}}
\newcommand{\jastp}{  {\it J. Atmos. Solar-Terr. Phys.}} 
\newcommand{\jgr}{    {\it J. Geophys. Res.}}
\newcommand{\mnras}{  {\it Mon. Not. Roy. Astron. Soc.}}
\newcommand{\nat}{    {\it Nature}}
\newcommand{\pasp}{   {\it Pub. Astron. Soc. Pac.}}
\newcommand{\pasj}{   {\it Pub. Astron. Soc. Japan}}
\newcommand{\pre}{    {\it Phys. Rev. E}}
\newcommand{\solphys}{{\it Solar Phys.}}
\newcommand{\sovast}{ {\it Soviet  Astron.}} 
\newcommand{\ssr}{    {\it Space Sci. Rev.}} 

%%%%%%%%%%%%%%%% Roadmap of the paper with all the labels %%%%%%%%%%%%%%%%%%%%%%%%
%%%% (with the exception of citations since author-year is easy to remember) %%%%%
1 Section~\ref{S-Introduction}
2 Section~\ref{S-general}
  Section~\ref{S-text}
  Section~\ref{S-labels}
3 Section~\ref{S-features}
  Section~\ref{S-equations}
   Section~\ref{S-simple-equations}
     Equation~(\ref{Eq-H-def})
   Section~\ref{S-array-equations}
     Equation~(\ref{Eq-A-B})
     Equation~(\ref{Eq-H-B})
     Equation~(\ref{Eq-H-N})
   Section~\ref{S-long-equations}
     Equation~(\ref{Eq-dH-Phi})  
  Section~\ref{S-figures}
  Section~\ref{S-tables}
  Section~\ref{S-references}
  Section~\ref{S-BibTeX}
  Section~\ref{S-Miscellaneous}
4 Section~\ref{S-Conclusion}

A Appendix~\ref{S-appendix}
 
 1 Figure~\ref{F-simple}
 2 Figure~\ref{F-4panels}
 3 Figure~\ref{F-rotate-cut}
 4 Figure~\ref{F-appendix}

 1 Table~\ref{T-simple}
 2 Table~\ref{T-complex}
 3 Table~\ref{T-appendix}

%%%%%%%%%%%%%%%%%%%% Results for the citation commands %%%%%%%%%%%%%%%%%%%%%%%%  
\cite{Kusano04}          : (Kusano \etal, 2004)
\cite{Kusano04,Berger03} : (Kusano \etal, 2004; Berger, 2003)
\inlinecite{Brown99}     : Brown, Canfield, and Pevtsov (1999)
\opencite{Brown99}       : Brown, Canfield, and Pevtsov, 1999
\citeauthor{Brown99}     : Brown, Canfield, and Pevtsov
\shortcite{Brown99}      : (1999)
\citeyear{Brown99}       : 1999
(\opencite{Berger84}, \citeyear{Berger03}) 
                         : (\opencite{Berger84}, \citeyear{Berger03})


